SPPL: Probabilistic Programming with Fast Exact Symbolic Inference

We present the Sum-Product Probabilistic Language (SPPL), a new probabilistic programming language that automatically delivers exact solutions to a broad range of probabilistic inference queries. SPPL translates probabilistic programs into sum-product expressions, a new symbolic representation and associated semantic domain that extends standard sum-product networks to support mixed-type distributions, numeric transformations, logical formulas, and pointwise and set-valued constraints. We formalize SPPL via a novel translation strategy from probabilistic programs to sum-product expressions and give sound exact algorithms for conditioning on and computing probabilities of events. SPPL imposes a collection of restrictions on probabilistic programs to ensure they can be translated into sum-product expressions, which allow the system to leverage new techniques for improving the scalability of translation and inference by automatically exploiting probabilistic structure. We implement a prototype of SPPL with a modular architecture and evaluate it on benchmarks the system targets, showing that it obtains up to 3500x speedups over state-of-the-art symbolic systems on tasks such as verifying the fairness of decision tree classifiers, smoothing hidden Markov models, conditioning transformed random variables, and computing rare event probabilities.

==> Makefile <==
.PHONY:all
all: clean submission

.PHONY:paper
paper:
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper

submission: paper
	pdftk paper.pdf cat 1-16 output pldi21main-p337-p.pdf
	pdftk paper.pdf cat 17-end output pldi21main-p337-p-appx.pdf

.PHONY:release
release: clean submission
	rm -rf pldi21main-p337-p.zip
	zip pldi21main-p337-p.zip \
		*.bib \
		*.bbl \
		*.tex \
		*.pdf \
		ACM-Reference-Format.bst \
		acmart-preload-hook.tex \
		acmart.cls \
		assets/* \
		figures/* \
		Makefile \
		README
	rm -rf pldi21main-p337-p-appx.zip
	zip pldi21main-p337-p-appx.zip pldi21main-p337-p-appx.pdf

.PHONY:clean
clean:
	rm -f *.out *.aux  *.bbl  *.log  *.bcf  \
		*.blg  *.log  *.xml  *.toc  *.gz  *.out  *.fls  *.fdb_latexmk  \
		*.snm *.nav pldi21main-p337-p* paper.pdf


==> acmart-preload-hook.tex <==
% See page of acmart.pdf documentation.
% https://www.latextemplates.com/svgnames-colors
\PassOptionsToPackage{svgnames}{xcolor}


==> figures/polynomial.tex <==
%!TEX root = ../paper.tex

\begin{figure*}[h]
\centering

\begin{subfigure}{\textwidth}
\centering
\begin{lstlisting}[style=sppl,frame=single,basicstyle=\ttfamily\normalsize]
X ~ normal(0, 2)
Z ~ -X^3 + X^2 + 6*X if (X < 1) else 5*sqrt(X) + 11
\end{lstlisting}
\begin{subfigure}[b]{.3\textwidth}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tikzpicture}
\Tree
  [.\node[circle,draw,inner sep = 1pt,](root){$+$};
    % Subtree.
    \edge node[auto=right]{.69};
    [.\node[name=t1, label={[name=t1l,label distance=.25cm]above left:{$({-\infty}, 1)$}}]{$X{\sim}{N}(0,2)$};
      \edge[-stealth,thick,color=red] node[auto=right,color=black]{$Z$};
      $-X^3{+}X^2{+}6X$ ]
    % Subtree.
    \edge node[auto=left]{.31};
    [.\node[name=t2,label={[name=t2l,label distance=.25cm]above right:{$(1,\infty)$}}]{$X{\sim}N(0,2)$};
      \edge[-stealth,thick,color=red] node[auto=right,color=black]{$Z$};
      $5\sqrt{X}{+}11$ ] ]
\draw[-stealth] (t1l) -- (t1);
\draw[-stealth] (t2l) -- (t2);
\end{tikzpicture}
\end{adjustbox}
% \vspace{.05cm}
\captionsetup{aboveskip=10pt, belowskip=0pt}
\caption{Prior Sum-Product Expression}
\label{subfig:poly-invert-prior-spe}
\end{subfigure}\hfill
\begin{subfigure}[b]{.7\textwidth}
\includegraphics[width=\textwidth]{assets/polynomial-0.pdf}
\captionsetup{aboveskip=-5pt, belowskip=0pt}
\caption{Prior Marginal Distributions}
\label{subfig:poly-invert-prior-dist}
\end{subfigure}
\end{subfigure}
% \hrule
\medskip

\begin{subfigure}{\textwidth}
\centering
\begin{lstlisting}[style=sppl,frame=single,basicstyle=\ttfamily\normalsize]
condition (Z^2 <= 4 and Z >= 0);
\end{lstlisting}
\begin{subfigure}[b]{.3\textwidth}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tikzpicture}
% \tikzset{level distance=2cm}
\tikzset{level 1/.style={level distance=2cm}}
\tikzset{level 2/.style={level distance=1.25cm}}
\Tree
  [.\node[circle,draw,inner sep = 1pt,](root){$+$};
    % Subtree.
    \edge node[auto=right]{.16};
    [.\node[name=t1,label={[name=t1l,label distance=.25cm]above left:$[-2.2,-2]$}]{$X{\sim}N(0,2)$};
      \edge[-stealth,thick,color=red] node[auto=right,color=black]{$Z$};
      $-X^3{+}X^2{+}6X$ ]
    % Subtree.
    \edge node[pos=.5, inner sep =.5pt, auto=right]{.49};
    [.\node[name=t2,label={[name=t2l,label distance=.15cm]above right:$[0,0.32]$}]{$X{\sim}N(0,2)$};
      \edge[-stealth,thick,color=red] node[auto=right,color=black]{$Z$};
      $-X^3{+}X^2{+}6X$ ]
    % Subtree.
    \edge node[auto=left]{.35};
    [.\node[name=t3,label={[name=t3l,label distance=.25cm]above right:$[3.2,4.8]$}]{$X{\sim}N(0,2)$};
      \edge[-stealth,thick,color=red] node[auto=right,color=black]{$Z$};
      $5\sqrt{X}{+}11$ ] ]
\draw[-stealth] (t1l) -- (t1);
\draw[-stealth] (t2l) -- (t2);
\draw[-stealth] (t3l) -- (t3);
\end{tikzpicture}
\end{adjustbox}
% \vspace{.01cm}
\captionsetup{aboveskip=15pt, belowskip=0pt}
\caption{Posterior Sum-Product Expression}
\label{subfig:poly-invert-post-spe}
\end{subfigure}\hfill
\begin{subfigure}[b]{.7\textwidth}
\includegraphics[width=\textwidth]{assets/polynomial-1.pdf}
\captionsetup{aboveskip=-5pt, belowskip=0pt}
\caption{Posterior Marginal Distributions}
\label{subfig:poly-invert-post-dist}
\end{subfigure}
\end{subfigure}
\hrule
\captionsetup{aboveskip=2pt,belowskip=0pt}
\caption{Inference on a stochastic many-to-one transformation of a real random variable in \sppl{}.}
\label{fig:poly-invert}
% \vspace{-.75cm}
\end{figure*}

